Robust Odometry and Mapping for Multi-LiDAR Systems with Online Extrinsic Calibration

Combining multiple LiDARs enables a robot to maximize its perceptual awareness of environments and obtain sufficient measurements, which is promising for simultaneous localization and mapping (SLAM). This paper proposes a system to achieve robust and simultaneous extrinsic calibration, odometry, and mapping for multiple LiDARs. Our approach starts with measurement preprocessing to extract edge and planar features from raw measurements. After a motion and extrinsic initialization procedure, a sliding window-based multi-LiDAR odometry runs onboard to estimate poses with online calibration refinement and convergence identification. We further develop a mapping algorithm to construct a global map and optimize poses with sufficient features together with a method to model and reduce data uncertainty. We validate our approach's performance with extensive experiments on ten sequences (4.60km total length) for the calibration and SLAM and compare them against the state-of-the-art. We demonstrate that the proposed work is a complete, robust, and extensible system for various multi-LiDAR setups. The source code, datasets, and demonstrations are available at https://ram-lab.com/file/site/m-loam.

==> biography.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/bio/jjh.png}}]{Jianhao Jiao}
received the B.Eng. degree in Instrument Science from Zhejiang University, Hangzhou, China, in 2017. 
He is currently pursuing the Ph.D. with the Department of Electronic and Computer Engineering, the Hong Kong University of Science and Technology, Hong Kong, 
China, supervised by Prof. Ming Liu. 

His research interests include state estimation, SLAM, sensor fusion, and computer vision.
\end{IEEEbiography}
\vspace{-0.3cm}

% if you will not have a photo at all:
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/bio/yhy.jpg}}]{Haoyang Ye}
received the B.Eng. in Automation from the College of Control Science and Engineering, Zhejiang University, Hangzhou, China, in 2016, 
and the Ph.D. from the Department of Electronic and Computer Engineering, the Hong Kong University of Science and Technology, Hong Kong, 
China, in 2020, supervised by Prof. Ming Liu.

His research interests include state estimation for robotics, SLAM, multi-sensor fusion, and robot navigation.
\end{IEEEbiography}
\vspace{-0.3cm}

% if you will not have a photo at all:
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/bio/zyl.jpg}}]{Yilong Zhu}
received B.Sc. in Instrument Science from Harbin institute of technology, China, in 2017, 
and the M.S degree in electrical engineering from the Hong Kong university of science and technology, China, 2018. 
He is currently pursuing the Ph.D in the same university, supervised by Prof. Ming Liu.

His research interests include SLAM, sensor fusion and preception.
He used to won the best paper finalist Award in 2019 IEEE International Conference on Robotics and Biomimetics. 
\end{IEEEbiography}
\vspace{-0.3cm}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/bio/ming.png}}]{Ming Liu}
received the B.A.
degree in automation from Tongji University, Shanghai, China, in 2005, and the Ph.D. degree from
the Department of Mechanical and Process Engineering, ETH Zurich, Z ¨ urich, Switzerland, in 2013, ¨
supervised by Prof. Roland Siegwart. 
During his master’s study with Tongji University, he stayed one year with the Erlangen-Nunberg University and ¨Fraunhofer Institute IISB, Erlangen, Germany, as a Master Visiting Scholar. He is currently with the Electronic and Computer Engineering, 
Computer Science and Engineering Department, Robotics Institute, The Hong Kong University of Science and Technology, Hong Kong, as an Associate Professor. 
%He is also a founding member of Shanghai Swing Automation Ltd., Co. He is coordinating and involved in NSF Projects and National 863-Hi-TechPlan Projects in China. 

His research interests include dynamic environment modeling, deep-learning for robotics, 3D mapping, machine learning, and visual control.

% Dr. Liu was a recipient of the European Micro Aerial Vehicle Competition (EMAV’09) (second place) and two awards from International Aerial Robot Competition (IARC’14) as a Team Member, the Best Student Paper Award as first author for MFI 2012 (IEEE International Conference on Multisensor Fusion and Information Integration), the Best Paper Award in Information for IEEE International Conference on Information and Automation (ICIA 2013) as first author, the Best Paper Award Finalists as co-author, the Best RoboCup Paper Award for IROS 2013 (IEEE/RSJ International Conference on Intelligent Robots and Systems), the Best Conference Paper Award for IEEE-CYBER 2015, the Best Student Paper Finalist for RCAR 2015 (IEEE International conference on Real-time Computing and Robotics), the Best Student Paper Finalist for ROBIO 2015, the Best Student Paper Award for IEEE-ICAR 2017, the Best Paper in Automation Award for IEEE-ICIA 2017, twice the innoviation contest Chunhui Cup Winning Award in 2012 and 2013, and the Wu Wenjun AI Award in 2016. He was the Program Chair of IEEERCAR 2016 and the Program Chair of International Robotics Conference in Foshan 2017. He was the Conference Chair of ICVS 2017.
% He has published many popular papers in top journals including IEEE TRANSACTIONS ON ROBOTICS (TRO) and INTERNATIONAL JOURNAL OF ROBOTICS RESEARCH (IJRR). Dr. Liu is currently an Associate Editor for IEEE ROBOTICS AND AUTOMATION LETTERS, IET CYBER-SYSTEMS AND ROBOTICS, INTERNATIONAL JOURNAL OF ROBOTICS AND AUTOMATION. He is a Senior Member of IEEE.
\end{IEEEbiography}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}



% that's all folks

==> exper_localization.tex <==
\subsection{Performance of Localization and Mapping}
\label{sec:exp_localization}

\begin{itemize}
	\item talk about the distinction: indoor (dominant planar features) and outdoor (have edged line and planar features) environment; simulation (have ground truth to qualify) and real sensor 
	\item RHD: 3 sequences: RHD\_room\_gt, RHD\_room\_wo\_gt, RHD\_campus\_wo\_gt, visualize the trajectory and RMSE, compare with other method
	\item RT: one sequence: RT\_bay\_gt, visualize the trajectory and RMSE, compare with other method
\end{itemize}


\begin{comment}
	\begin{table}[]
	\centering
	\caption{RMSE \cite{} in all simulated and real sequences.}
	\renewcommand\arraystretch{1.25}
	\renewcommand\tabcolsep{3pt}	
	\begin{tabular}{cccc}
	\hline
	\toprule[0.03cm]
	Sequence  & LOAM & M-LO & M-LOAM \\ 
	\hline
	\toprule[0.01cm]		
	SR01easy      &      &        &      \\ 
	SR02easy      &      &        &      \\ 
	SR03medium    &      &        &      \\ 
	SR04medium    &      &        &      \\ 
	SR05difficult &      &        &      \\ 
	\hline
	\toprule[0.01cm]		
	RHD02         &      &        &      \\ 
	RHD03         &      &        &      \\ 		
	\hline
	\toprule[0.01cm]		
	RT02          &      &        &      \\ 
	\hline
	\toprule[0.03cm]		
	\end{tabular}
	\label{table.rmse}
	\end{table}
\end{comment}
